Pose-independent 3D Anthropometry from Sparse Data

3D digital anthropometry is the study of estimating human body measurements from 3D scans. Precise body measurements are important health indicators in the medical industry, and guiding factors in the fashion, ergonomic and entertainment industries. The measuring protocol consists of scanning the whole subject in the static A-pose, which is maintained without breathing or movement during the scanning process. However, the A-pose is not easy to maintain during the whole scanning process, which can last even up to a couple of minutes. This constraint affects the final quality of the scan, which in turn affects the accuracy of the estimated body measurements obtained from methods that rely on dense geometric data. Additionally, this constraint makes it impossible to develop a digital anthropometry method for subjects unable to assume the A-pose, such as those with injuries or disabilities. We propose a method that can obtain body measurements from sparse landmarks acquired in any pose. We make use of the sparse landmarks of the posed subject to create pose-independent features, and train a network to predict the body measurements as taken from the standard A-pose. We show that our method achieves comparable results to competing methods that use dense geometry in the standard A-pose, but has the capability of estimating the body measurements from any pose using sparse landmarks only. Finally, we address the lack of open-source 3D anthropometry methods by making our method available to the research community at https://github.com/DavidBoja/pose-independent-anthropometry.

==> tables/caesar-standing-results.tex <==
\begin{table}[h!]
\scriptsize
\begin{center}
\caption{MAE results on the CAESAR standing subjects in mm. We abbreviate the measurements as: Circumferences (C.), Heights (H.) and Lengths (L.).}
%\rowcolors{2}{blue!10}{white}
% ZA MAX LM DIST OD 5.64836198464036 mm
% ankle left circumference 	 2.62mm
% arm length (shoulder to elbow) 	 1.28mm
% arm right length 	 4.04mm
% arm length (spine to wrist) 	 3.17mm
% chest circumference 	 15.52mm
% crotch height 	 2.37mm
% head circumference 	 1.56mm
% Hip circumference max height 	 1.49mm
% hip circumference 	 7.08mm
% neck circumference 	 1.67mm
% height 	 2.52mm
\begin{tabular}{|l|c|c|c|c|c|c||c|c|c|c|c|c|c|c|}
\cline{2-13}
      \multicolumn{1}{c|}{}     & \multicolumn{6}{c||}{MALE}           & \multicolumn{6}{c|}{FEMALE}    &    \multicolumn{1}{|c}{} \\
\cline{2-14}
      \multicolumn{1}{c|}{}     & \multicolumn{3}{c|}{dense data}           & \multicolumn{3}{c||}{sparse data}    &  \multicolumn{3}{c|}{dense data}           & \multicolumn{3}{c|}{sparse data} &  {\tiny AE} \\  \hline
{\tiny Measurem.}              & \cite{anthroscan} & \cite{scan-db} & \cite{tsoli-mode-based-anthropometry} & baseline & \cite{bojanic_VISAPP24} & Ours & \cite{anthroscan} & \cite{scan-db} & \cite{tsoli-mode-based-anthropometry} & baseline & \cite{bojanic_VISAPP24} & Ours  & {\tiny \cite{AE}} & {\tiny Ambig.} \\ \hline
{\tiny Ankle C. }     & 13.66   & 5.72    & 5.56 &  23.62   & 6.24 & 6.06         & 7.55    & 6.59    & 6.19 &  17.55   & 5.87 & 6.73 & 4     & 2.62     \\ \hline
\makecell[cl]{ \tiny Shoulder to \\ \tiny elbow L.} & 13.99   & 12.66   & 13.32 & 36.50   & 6.95 & 8.19          & 11.26   & 8.42    & 6.65 & 33.67    & 6.32 & 7.66 & 6   & 1.28       \\ \hline
{\tiny C} & 14.49   & 13.76   & 12.66 & 55.81   & 9.93 & 10.02          & 11.67   & 10.42   & 10.05 & 49.80   & 7.36 & 8.52 & -  & 4.04    \\ \hline
{\tiny D }  & 14.71   & 11.81   & 10.40 & 45.21   & 11.38 & 13.06          & 13.19   & 13.40   & 11.87 & 41.74   & 9.84 & 10.95 & -   & 3.17       \\
{\tiny E  }    & 13.96   & 15.21   & 13.02 & 73.91   & 18.24 & 22.50         & 12.43   & 13.02   & 12.73 & 41.52   & 17.26 & 20.45 & 15    & 15.52     \\
{\tiny F} & 11.01   & 9.77    & 8.36 & 17.65    & 1.17 & 6.74       & 7.45    & 7.53    & 5.50 & 13.85    & 0.78 & 5.38 & 10     & 2.37    \\
{\tiny G   }    & 5.51    & 7.46    & 5.59 & 21.93    & 8.92 & 9.73        & 7.44    & 7.45    & 5.91 & 16.81    & 8.42 & 10.73  & 5     & 1.56     \\
{\tiny H } & 16.50   & 18.89   & 19.05 & 26.41   & 17.33 & 19.26        & 17.05   & 18.96   & 18.59 & 36.34   & 20.99 & 20.39 & -    & 1.49      \\
{\tiny I  }      & 7.90    & 12.57   & 10.66 & 46.51   & 22.87 & 21.89         & 7.47    & 16.15   & 12.35 & 40.06   & 21.40 & 21.29 & 12   & 7.08      \\
{\tiny J } & 21.57   & 13.33   & 13.47 & 74.15   & 12.40 & 16.87         & 21.03   & 16.35   & 15.43 & 88.31   & 13.84 & 14.55 & 11  & 1.67       \\
{\tiny K }               & 5.86    & 7.98    & 6.53 & 14.00    & 5.75 & 11.13         & 5.60    & 10.21   & 7.51 & 25.69    & 5.52 & 8.92  & 10 & 2.52        \\ \hline \hline 
{\tiny aMAE}                     & 12.65   & 11.74   & 10.78 & 39.61   & 11.02 & 13.22          & 11.10   & 11.68   & 10.25 & 36.85   & 10.69 & 12.32 &            \\ \hline       
\end{tabular}
\end{center}
\end{table}
